The trade-offs of model size in large recommendation models : A 10000 $\times$ compressed criteo-tb DLRM model (100 GB parameters to mere 10MB)

Embedding tables dominate industrial-scale recommendation model sizes, using up to terabytes of memory. A popular and the largest publicly available machine learning MLPerf benchmark on recommendation data is a Deep Learning Recommendation Model (DLRM) trained on a terabyte of click-through data. It contains 100GB of embedding memory (25+Billion parameters). DLRMs, due to their sheer size and the associated volume of data, face difficulty in training, deploying for inference, and memory bottlenecks due to large embedding tables. This paper analyzes and extensively evaluates a generic parameter sharing setup (PSS) for compressing DLRM models. We show theoretical upper bounds on the learnable memory requirements for achieving $(1 \pm \epsilon)$ approximations to the embedding table. Our bounds indicate exponentially fewer parameters suffice for good accuracy. To this end, we demonstrate a PSS DLRM reaching 10000$\times$ compression on criteo-tb without losing quality. Such a compression, however, comes with a caveat. It requires 4.5 $\times$ more iterations to reach the same saturation quality. The paper argues that this tradeoff needs more investigations as it might be significantly favorable. Leveraging the small size of the compressed model, we show a 4.3$\times$ improvement in training latency leading to similar overall training times. Thus, in the tradeoff between system advantage of a small DLRM model vs. slower convergence, we show that scales are tipped towards having a smaller DLRM model, leading to faster inference, easier deployment, and similar training times.

==> tables/t0.tex <==
\begin{table}[]
\caption{Time taken for original embedding table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|cccccccl|}
\hline
\multicolumn{8}{|c|}{\textbf{Original time(ms)}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textit{}}}     & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} }}                & \multicolumn{6}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{n}}}                                                                                                                                                                                                                                                                                                                              \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{call}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} \textbf{sparse}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 4M}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 8M}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 16M}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 32M}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} 64M}} & {\color[HTML]{333333} 128M} \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}backward}                             & \multicolumn{1}{c|}{\cellcolor[HTML]{F4F6F8}FALSE}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FCCB67}25.68}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{F9C069}50.72}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{F3A96C}100.72}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{E67C73}200.67}                     & \multicolumn{1}{c|}{\cellcolor[HTML]{EA4335}}                           & \cellcolor[HTML]{EA4335}    \\ \hline
\rowcolor[HTML]{FFD666} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}}                                     & \multicolumn{1}{c|}{\cellcolor[HTML]{F4F6F8}TRUE}                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFD666}0.35}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFD666}0.35}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFD666}0.38}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFD666}0.38}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{FFD666}0.35}                       & \cellcolor[HTML]{EA4335}    \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}forward}                              & \multicolumn{1}{c|}{\cellcolor[HTML]{F4F6F8}FALSE}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{B5CA76}0.21}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{B7CA76}0.22}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{BCCB75}0.22}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{BCCB75}0.22}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{EA4335}}                           & \cellcolor[HTML]{EA4335}    \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}}                                     & \multicolumn{1}{c|}{\cellcolor[HTML]{F4F6F8}TRUE}                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{59BB8A}0.12}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{59BB8A}0.12}                      & \multicolumn{1}{c|}{\cellcolor[HTML]{59BB8A}0.12}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{57BB8A}0.12}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{57BB8A}0.12}                       & \cellcolor[HTML]{EA4335}    \\ \hline
\end{tabular}
}
\vspace{-0.8cm}
\label{tab:t0}
\end{table}

==> tables/t9.tex <==
\begin{tabular}{|ccccc|}
\hline
\multicolumn{5}{|c|}{\textbf{Forward pass (ms) {[}sparse=false{]}}}                                                                                                                                                                                                                                                           \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textit{}}      & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{compression}}                                                                                                                                                                                              \\ \hline
\rowcolor[HTML]{FFFFFF} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{chunk}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 10x}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 100x}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{000000} 1000x}} & {\color[HTML]{000000} 10000x} \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}1}              & \multicolumn{1}{c|}{\cellcolor[HTML]{E98671}0.89}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{E88272}0.90}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{F3AA6C}0.73}                         & \cellcolor[HTML]{5DBC89}0.28  \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}2}              & \multicolumn{1}{c|}{\cellcolor[HTML]{F1A36D}0.77}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{EF9C6E}0.80}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FBC768}0.61}                         & \cellcolor[HTML]{57BB8A}0.27  \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}4}              & \multicolumn{1}{c|}{\cellcolor[HTML]{F9BE69}0.65}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{F9BE69}0.65}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FED567}0.54}                         & \cellcolor[HTML]{58BB8A}0.27  \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}8}              & \multicolumn{1}{c|}{\cellcolor[HTML]{A4C77A}0.40}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{A2C77A}0.39}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{77C084}0.32}                         & \cellcolor[HTML]{5EBC89}0.28  \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}16}             & \multicolumn{1}{c|}{\cellcolor[HTML]{96C57D}0.37}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{96C57D}0.37}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{6BBE86}0.30}                         & \cellcolor[HTML]{62BC88}0.29  \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{F4F6F8}32}             & \multicolumn{1}{c|}{\cellcolor[HTML]{94C47D}0.37}                       & \multicolumn{1}{c|}{\cellcolor[HTML]{92C47E}0.37}                        & \multicolumn{1}{c|}{\cellcolor[HTML]{6DBE86}0.30}                         & \cellcolor[HTML]{6BBE86}0.30  \\ \hline
\end{tabular}

==> text/Introduction1.tex <==
% Recommendation systems are an essential key challenge in embedding tables. 
Recently, recommendation systems have emerged as one of the largest workloads in machine learning \cite{archimpl}. Recommendation systems form the backbone of good user experience on online platforms such as e-commerce and web search, where there is a flood of information. Thus, considerable effort goes into building recommendation systems. Deep learning recommendation models give state-of-the-art performance. However, recommendation models suffer from a critical challenge - sparse features with millions of categorical values. \cite{DLRM19, mudigere2021high} These state-of-the-art \cite{DLRM19, DCN17, song2019autoint, guo2017deepfm, huang2019fibinet, lian2018xdeepfm} methods learn a dense representation of the categorical values in a parameter structure called {\em embedding table}.

% Recommendation models are significant due to embedding tables. n blows up. Efforts have been put into finding compressed representations for embedding tables. One of the most eye-opening results has been ROBE-Z. 

Industrial-scale recommendation models are one of the largest models built, and the size of the embedding table can go as large as hundreds of terabytes. For example, a research article from Facebook discusses the training of a model of size 50TB over 128 GPUs \cite{mudigere2021high}. More than 99.9\% of the model memory is occupied by embedding tables in these models. The scale of these models leads to a plethora of other problems - slower inference time, slower training time per iteration, significant engineering challenges in training. In light of these issues, many works have investigated learning of compressed representation of embedding tables using various principles such as compositional embeddings \cite{QuoRemTrick19}, exploiting power-law in the observed frequencies of tokens \cite{MDTrick19, md1,md2,md3,md4,md5}, low-rank decomposition \cite{ttrec}, and weight sharing methods \cite{robez}. An excellent summary of related compression work is presented in section 2 of \cite{robez}. Also, a summary of state-of-the-art results is presented in table 3 of \cite{robez}. We direct the readers to refer to these pieces from \cite{robez} and avoid discussing these in this paper in the interest of space. The state-of-the-art compression method of Random Offset Block Embedding (ROBE) array \cite{robez} shows compression of 1000$\times$ for criteo-tb dataset without loss of quality. This method outperforms all the contending approaches by order of magnitude more compression. Parameter sharing methods such as ROBE will be the focus of our paper.

% Downplay robe-z. Say it does something. While training times are supposed to improve, they do not. Compression factor evaluation is incomplete. We improve the ROBE-Z implementation to gain significant improvement in training time per iteration. We also perform a rigorous evaluation of ROBE-Z to understand the intricate details and present them in section .. as a guideline for running ROBE-Z.

The results presented in \cite{robez} are eye-opening. They point out the number of excess parameters in recommendation systems. They also show how achieving 1000$\times$ compression leads to improvement in inference throughput. They discuss the downside of training compressed model in terms of slower convergence, and they could not show improved training time per iteration or did not make any conclusive comment on overall training time. This line of work raises many questions about state-of-the-art recommendation systems. Specifically, it stands to reason that we need to investigate the value of excess parameters in the recommendation system. We seek to understand the answers to the following research questions in this paper.
% This has opened up many questions. (1) how small can embedding tables go? Empirical evaluation. Any guide from the theory? (2) How does the reduction in excess parameters affect convergence, and when is it, if at all, compensated by improvement in training time iterations. In general, we are trying to understand the implications of "excess parameters" in recommendation models where excess parameter influx happens in embedding tables. 
\begin{figure}
        \centering
        \caption{This not-to-scale illustration shows tradeoffs of having larger parameters ( and hence memory footprint of the model ). Each line has its own scale. As we move towards the right, memory increases, and we need to have memory farther away from computational hardware. This increases the latency and thus inference time and training time per iteration. The energy cost also increases due to larger active hardware. We observe that the convergence becomes faster as the number of parameters increases. The solid lines show the overall training time and training costs, and it shows that more parameters are not always better.}   
    \includegraphics[scale=0.16]{fig/tradeoff2.png}
    \vspace{-0.5cm}
     \label{fig:tradeoff}
\end{figure}
\begin{enumerate}[leftmargin=*, nosep]
    \item What is the extent of compression that can be obtained in embedding tables using parameter sharing setups. Is there any theoretical basis for this compression?
    \item Is the increase in the number of iterations for convergence compensated by the improvement in training time per iteration. How to realize a better training time per iteration? In the process, also figure out the settings in which PSS works best using ROBE-Z as a case study.
\end{enumerate}
We summarize our findings below,

\textbf{Compression of embedding tables:} We formulate a general parameter sharing setup (PSS) for embedding tables which approximate an embedding table $E \in R^{n \times d}$  up to a factor of $\epsilon$. These are called as $(1 \pm \epsilon)$ PSS for E (exact definition in section \ref{sec:theory}) . We present a Johnson-Lindenstrauss transform (JLT) based PSS, which are provable $(1 \pm \epsilon)$ PSS. For example, using a standard normal JLT we can obtain a $(1 \pm \epsilon)$ PSS using $\mathcal{O}(\sigma^2(E) / \epsilon^2 ( log(1/\delta) + \max(d^2, d.log(n)) )$ parameters with a probability of $(1 - \delta)$. Here $\sigma(E)$ denotes the maximum singular value of E. This logarithmic dependence on $n$ is encouraging as the primary reason for the blow up of embedding table size comes from huge values of $n$ while $d$ is generally restricted to a few hundred. Intuitively, one can expect a large compression, as the blow up in parameters, is an inadvertent effect of naively building embedding tables .
%where the value of embedding tables, arguably, is to capture the relations between different tokens in dense space.  (this is under selling the theory later) so remove
ROBE-Z can also be explained in this framework. This relation is explained in section \ref{sec:robez}

Our theory makes us wonder if even more compression is possible with a $(1 \pm \epsilon)$ PSS for E. To our astonishment, we can achieve \textbf{10,000 $\times$ compression for criteo-tb} dataset (an order of magnitude higher than compression reported by \cite{robez}) without any loss of quality. That is, using only \textbf{10MB} of embedding parameters, we can achieve results of original \textbf{100GB} of parameters. More importantly, this comes at \textbf{minimal increase of 1.04 $\times$ in overall training time}, not to mention the improvement in inference time and energy cost savings. This level of compression without any adverse effects is unprecedented in the embedding table compression research.

\textbf{Training time for learning $(1 \pm \epsilon)$ PSS: }
As a general observation, if the number of parameters in the model is large, then the convergence is faster. This has been proved for some cases with overparameterized DNNs \cite{allen2019convergence}. In our experiments, we observe that as the number of parameters in the model is reduced, by using a PSS in this case, the number of iterations required to converge to target quality increases. This is a concern since training times are one of the major aspects of the model. However, when we compress the model such that it completely changes the way embedding table parameters are stored ( for example, from multiple nodes to single node, from RAM to GPU, or multiple GPUs to single GPU ), there is going to be a steep decrease in the latency of embedding lookup/gradient update operations. The question of how this improvement in latency compensates for increased training iterations is worth investigating. We implement an optimized version of ROBE-Z minimizing data movement costs, implementing sparse and dense gradient propagation in ROBE-Z and simplifying the
original code immensely. We detail these efforts in section \ref{sec:robez_exp}. We compare the overall training times of the different sized PSS with original model training for the criteo-tb dataset and find that the training times do not suffer much. For example a 1,000$\times$ compressed model trains in $1.1 \times$ time whereas a 10,000$\times$ compressed model trains at $1.04 \times$ time as compared to original model.  These results are presented, along with other results on inference time, etc., in section \ref{sec:results}. We also perform additional evaluation of ROBE-Z with different settings of the chunk size, size of embedding tables, compression rates, and dense/sparse gradient propagation in section \ref{sec:robez_exp} which will provide a guideline to obtain maximum benefit from PSS like ROBE-Z. 

\textbf{System tradeoffs of the excess number of parameters:}As a general message, there are four critical aspects of models: (1) inference time, (2) training time, (3) energy costs of training, and (4) engineering challenges in training and deployment. Figure \ref{fig:tradeoff} illustrates these different factors and how they change with the increase excess parameters. As the memory usage increases, the model has to be stored in more complicated setups affecting the latency of memory access and increasing the training time per iteration and inference times. Also, the cost of training increases due to more active hardware. However, arguably one of the good effects of having more parameters (beyond the minimum required) is the number of iterations required to converge to the target quality. The "iterations to converge vs. memory" profile predominantly affects the best (optimal) number of excess parameters in the system. For example, if the grey region in figure \ref{fig:tradeoff}, which defines the minimum required parameters, extends into multi-node memory, then we have no choice but to run a distributed setup for model training/inference. However, if the minimum required parameters lie in smaller memory zones like shown in figure \ref{fig:tradeoff}, then we might be able to achieve much smaller models that are better on all four aspects - better inference time, better training times, better cost of training, and no engineering challenges. In such a case, there seems to be no value in the excess parameters in the model. On the flip side, excess parameters lead to slower inference and higher costs. In our experience with the criteo-tb dataset, this is precisely the case.

==> text/abstract.tex <==

Recommendation models comprise more than 70\% of AI inference cycles in the cloud. The most popular MLPerf benchmark - Deep learning based recommendation models (DLRM) model consist of over 100 GB (25+ billion parameters), which is trained on terabytes of click through data. 
%Most commercial recommendation systems consider this public benchmark closest to real recommendation systems that are deployed in practice.  
 %achieve state-of-the-art performance in recommendation systems. Industrial-scale DLRMs are among the biggest models and learn a dense embedding for the pervasive categorical values in recommendation data. A large number of categorical values is a primary reason behind the explosion of parameters in DLRM. 
 DLRMs due to its sheer size and the associated volume of data face difficulty in training, deploying for inference, and memory bottlenecks due to large embedding tables. %Thus, substantial efforts have gone into embedding compression research. %In recently published ROBE \cite{robez}, authors demonstrated 1000$\times$ compression of embedding tables in a criteo-tb dataset without loss of quality. 
 This paper analyzes and extensively evaluates a generic parameter sharing setup (PSS) for compressing DLRM models. We show theoretical upper bounds on the memory requirements for achieving $(1 \pm \epsilon)$ approximations to embedding table. Our bounds indicate exponentially less parameters suffice for good accuracy. To this end, we show a scheme which does reach 10000$\times$ compression without losing quality. Such compression however comes with a compromise. It requires 4 times more epochs to reach the same saturation accuracy. In this paper, we argue that this trade-off needs more investigations as it might be significantly favorable. Higher compression while maintaining quality positively affects many factors - memory, inference time, and deployment complexity except, arguably, only one - training time.
 %In \cite{robez}, authors did not show any improvements in training time per iteration. 
 %We extensively test and show that compression can also improve training time per iteration. 
 %We can achieve 10000$\times$ compression without any serious penalty on overall training time (within 5-10\%). 
 We analyze the tradeoff between system-advantage of having higher compression vs. faster convergence of original embedding and conclude that higher compression maintaining quality leads to better models in all aspects, including training, and has seemingly no downside. 
 
 


==> text/introduction.tex <==
[intro has parts of robe-z paper]
There are generally 4 important aspects of models. 
1) training time for obtaining a specific quality of model
    - number of iterations
    - training time per iteration.
2) inference time with this model.
3) engineering challenges in training the model
4) quality of the model reached.

Over-parameterizing the models have become a norm for its fast convergence properties. However, the general effect of having excess parameters is known to have adverse effects on other three aspects of machine learning models. This gets especially cumbersome in case of DLRM models where the most obvious model already leads to TB sized models. ROBE-Z gives a clean and system-friendly way to reduce these excess parameters. We measure the effect of reduction in excess parameters 
While generally large models are good for generalization (and hence quality of model) and fast-convergence and that itself is good enough grounds for over-parameterization even though it affects inference time, training time per iteration and engineering effort adversely. However, the burden of over-parameterization / excess parameters in the system is immense and this is quite apparent in the DLRM models where most obvious way to get a model already has TB sized models. These large models cause have especially adverse effects on other three parameters. As we shall see in this paper 

\paragraph{Conclusions in the paper}: 
1) with robe-z we can control excess parameters in a nice clean and system-friendly way
2) The excessive burden of large model can be brought down significantly - as large as 10,000x without any loss of quality of the model. \textbf{This is the first time such results have been showcased on Criteo TB dataset} 
3) With high compression like 10,000x, there is immense improvement in inference time of the model. 
4) with high compression like 10,000x, there is significant ease of training DLRM models accessible to a general researcher.
5) with high compression like 10,000x, there is a significant reduction of training time per iteration. 
6) The increase in number of iterations for convergence that comes with reduction of excess parameters is largely offset by the decrease in the training time per iteration. So, overall in order to train a 10000x small model on a single GPU is only 1.2 $\times$ the time taken for training original DLRM model on criteo TB.
The conclusion is - it is not worth having excess parameters in recommendation models. 
Yes fast convergence - at what cost? 

\paragraph{Case study of DLRM models. }
Theoretical questions. 
1) How small can memory go? when does model starts loosing accuracy ?
For a specific requirement of preservation of inner products of the form $e_i E x$, we can show that this happens with probability (1- $\delta$ when memory is of the $O(\frac{1}{\epsilon^2}d log(\frac{9^d + n}{\delta}))$ The theorem follows from the l2-subspace embedding literature applied to a column space of $E$ and $n$ one-hot encoding vectors. Preservation of norms naturally lead to preservation of inner products. We learn the subspace embedding directly which ensures preserving of inner products. This is an existence proof explaining why it can happen that . Whether SGD is able to learn this l2-subspace embedding is an interesting question to which we cannot provide an answer at this point.

2) can we explain why number of training epochs is larger with higher compression.


Message: Value of excess parameters in large scale systems : Possibly very low.
1. Recommendation models are large by nature of their construction. How many excess parameters does it contain? How small can we go?
2. Empirically smaller models lead to slower convergence. However it also means more distributed setup and slower iteration times. Does having a compressed model eliminating engineering complexities still at any disadvantage to larger models?

Clearly, you can get improved performance from deep learning if you use more computing power to build bigger models and train them with more data.
overparameterization + SGD is the key?


==> text/theory.tex <==
\label{sec:theory}
\subsection{Introduction to parameter sharing setup} 
We will start this section by describing the parameter sharing setup for embedding tables. For simplicity, let us assume that we have a single embedding table $E \in R^{n \times d}$. A parameter sharing embedding setup consists of a set of weights $M$ and a recovery function $\mathcal{M}$. The memory $M$ can be organised in any manner suitable (example single array , 2D array etc). We denote the number of weights in $M$ by $|M|$. The recovery function returns an embedding of dimension $d$ for any integer in range $\{0,..,n-1\}$ given memory $M$. We can write,

\begin{equation}
\mathcal{M} : R^{|M|} \times \{0,..,n-1\} \rightarrow R^{d}
\end{equation}
Storing this mapping also requires some memory and we write this explicitly as $|\mathcal{M}|$. The purpose of parameter shared embeddings is to find a $(M,\mathcal{M})$ such that $(|M| + |\mathcal{M}|) \ll nd$ and the quality of embeddings is similar to that given by a full fledged embedding table $E$. 
Before we proceed to formalize the ``quality of embeddings", we would like to make a short comment on the choices of $|M|$ and $\mathcal{M}$.
\paragraph{$\mathbf{M}$ and $\mathbf{\mathcal{M}}$}
Note that we can make $M$ large in order to simplify $\mathcal{M}$. For example if $M = E$ then $\mathcal{M}(M, i) = M[i]$. On the other hand we can have only two weights of 0 and 1 in M and include all the complexity of embedding tables into mapping which first generates the binary representations of the embedding values from 0 and 1 and then outputs the values. However, one can imagine that these setups are not very useful. In fact in the context of training and inference with parameter shared embedding setups, it would be reasonable to make the following goals : (a) learnable memory M. (b) differentiable function $\mathcal{M}$ (c) $|\mathcal{M}|$ small as we want to invest most of available memory into learnable $M$. (d) Cheap computation cost of $\mathcal{M}$ over $M$. We will show a construction of such a setup in later part of this section.

Let us now talk about the goodness of parameter shared setup for any given embedding table $E \in R^{n \times d}$. We want to `simulate' the embedding table $E$ with parameter shared setup $(M, \mathcal{M})$. It is easy to prove that we cannot have a parameter shared setup of size sublinear in $nd$ to solve the exact problem of $\mathcal{M}(M,i) = E[i] \forall i \in \{0,..n-1\}$. Hence, we define approximate condition. We first state the condition and then elaborate on this choice.

\begin{definition}[${\epsilon}{-}l_2$ setup]
    A setup $(M, \mathcal{M})$ is called as an ${\epsilon}{-}l_2$ setup for an embedding table E if the following holds 
    \begin{align}
        & \forall x \in R^d \; \forall i \in \{0,..,n{-}1\} \;\\
        & \quad | \langle \mathcal{M}(M,i) , x \rangle - \langle E[i], x \rangle | \leq \epsilon ||x||_2
    \end{align}
    where $0 < \epsilon < 1$.
\end{definition}

The formulation of ${\epsilon}{-}l_2$ setup comes from the observation that we usually use embeddings in the following manner $\langle E[i], x \rangle$ for some i and some vector x (generally the weight vector from model that follows embedding tables. Thus there is value in trying to maintain these inner products. Note that the ${\epsilon}{-}l_2$ setup also preserves the inner products between pairs of embedding themselves. We state this as a lemma,
\begin{lemma}
If $(M, \mathcal{M})$ is a ${\epsilon}{-}l_2$ setup of embedding table E, then 
\begin{equation}
    | \langle \mathcal{M}(M, i) , \mathcal{M}(M, j) \rangle -  \langle E[i], E[j] \rangle | \leq 3\epsilon ||E[i]||_2 ||E[j]||_2
\end{equation}
\end{lemma}
\begin{proof}
By applying the ${\epsilon}{-}l_2$ twice, we can prove that,
\begin{align}
& (1-\epsilon)^2 || E[i]||_2 || E[j] ||_2 \leq \langle \mathcal{M}(M, i) , \mathcal{M}(M, j) \rangle\\
&\langle \mathcal{M}(M, i) , \mathcal{M}(M, j) \rangle \leq (1+\epsilon)^2 || E[i]||_2 || E[j] ||_2
\end{align}
which leads to the result.
\end{proof}

Thus being a  ${\epsilon}{-}l_2$ setup is a stronger condition than just preserving pairwise inner products among embeddings. Also, the definition of ${\epsilon}{-}l_2$ setup is geared towards making sure that the subsequent training works. 

\subsection{Upper bound on memory of ${\epsilon}{-}l_2$ setup for E}
In this section, we prove an upper bound for the memory of ${\epsilon}{-}l_2$ setup. We give a construction of M and $\mathcal{M}$ such that $|M|$ is $\mathcal{O}(d.max(log(n), d))$ and $|\mathcal{M}|$ which is $\mathcal{O}(1)$. We leverage the rich literature on Johnson-Lindenstrauss transforms (JLT) \cite{} and state our construction in terms of a JLT transform. This will allow practitioners to freely choose $S$ from the literature. We will also discuss a specific JLT transform that requires only $O(1)$ memory to store 
We will use the following definition 3 of JLT transforms from \cite{woodruff}. To paraphrase, a random matrix $S \in R^{k\timesn}$ is a $JLT(\epsilon,\delta,f)$ transform with parameters $\epsilon, \delta, f$ if with probability at least $(1-\delta)$ for any f-element subset $V \subset R^n$, the following holds for all $v_1, v_2 \in V$
\begin{equation}
    |\langle Sv_1, Sv_2 \rangle - \langle v_1, v_2 \rangle | \leq \epsilon || v_1 ||_2 || v_2 ||_2
\end{equation}

\begin{theorem} \label{th:1}
    Given an embedding table E. Consider a matrix S which is JLT($\epsilon/\sigma(E), \delta, (9^d + n)$ where $\sigma(E)$ denotes the maximum singular value of E. Then M and $\mathcal{M}$ defined as 
    \begin{equation}
        M = SE
    \end{equation}
    \begin{equation}
        \mathcal{M}(M, i) = (SE)^\top S e_i
    \end{equation}
    where $e_i\in R^n$ is a one-hot encoded vector of $i$ in $R^n$. Then (M,$\mathcal{M}$)  is a $l_2{-}\epsilon$ setup for E.
\end{theorem}
\begin{proof}
Proof can be found in appendix. \textit{Sketch:} We essentialy look at the set  $\{e_1, e_2, ..., e_n\} \cup 1/2-net(CS(E))$ where CS(E) denotes the column space of E. Total number of points in this set are $(9^d + n)$. Then we just want to preserve inner products among vectors in this set. Using properties of JLT for this space, we can prove the above theorem.
\end{proof}

We can apply theorem \ref{th:1} to obtain good ps-setups for embedding tables. \textbf{TODO}  talk about normal S . Its memory to store M and mapping. $\mathcal{M}$. Then discuss count sketch S. Its memory and M and mapping. End the section with a theorem for normal and count sketch matrices.

\subsection{Learning a $\epsilon-l_2$ setup}

==> text_nips/robez.tex <==
\input{tables/sota}
In this section, we will briefly review practical relaxations of PSS defined above. 

\textbf{Sparse JL with independence relaxation:} The issue with storage costs of S can be alleviated in practice by relaxing the complete independence condition on entries of S. For example, the JLT matrix (which requires same bound on k as given in \ref{thm:2}) suggested by \cite{achlioptas2003database}, which selects each entry to be 0 with probability 2/3 , $\pm 1$ with probability 1/6 independently can be generated on-the-fly using universal hashing. \cite{mitzenmacher2008simple} analyse why simpler hash functions can work well with data having enough entropy. The benefit of using universal hashing is that mapping $\mathcal{M}$ can now be stored in $O(1)$ memory. Thus using the \cite{achlioptas2003database} sparse matrix, we can obtain $(1 \pm \epsilon)$ PSS using total setup memory of  $|M| + |\mathcal{M}| =\mathcal{O}(1/\epsilon^2 \max(d^2, d.log(n)) )$ and cost of applying mapping $\mathcal{M}$ to be $\mathcal{O}(d)$ (hash computation and lookups) under valid independence relaxation.

Existing parameter-sharing based embedding compression methods can also be seen as PSS with varied distributions over S. We state a few of them below.
\begin{itemize}[nosep, leftmargin=*]
    \item \textbf{Hashing Trick} In this method, entire embeddings for a token $i$ is drawn from a randomly hashed location. In terms of PSS, we can define the mapping function $\mathcal{M}_h$ over a 2D matrix $\mathcal{M}_h \in R^{k \times d}$ where $k < n$.
    \begin{equation*}
    \mathcal{M}_h(M_h, i)[:] =  M_h[h(i), :]
    \end{equation*}
    where h is a hash function.
    \item \textbf{QR decomposition}\cite{QuoRemTrick19}. In this method, embedding for a token $i$ is drawn in chunks from separate memory vectors. In terms of PSS, we can define the mapping function $\mathcal{M}_q$ over, say l, pieces of 2D memory $M_1, M_2, .. M_l \in R^{k \times {d/l}}$ as follows
    \begin{equation}
        \mathcal{M}_q(\{M_1,M_2,..M_k\}, i)[j*(d/l):(j+1)*(d/l)] = M_j[h_j(i)]
    \end{equation}
    In words, the $j^{th}$ chunk of $i^{th}$ embedding is recovered using the chunk at the location $h_j(i)$ in memory $M_r$
    
    
    
    \item \textbf{ HashedNet~\cite{hashtrick} and ROBE-Z~\cite{robez} }: In HashedNets, authors proposed mapping model weights randomly into a parameter array. ROBE-Z extended this idea by hashing chunks of embedding vector instead of individual elements. In terms of PSS, we can define the mapping function $\mathcal{M}_r$ over 1D memory $M_r$ as
    \begin{equation*}
    \mathcal{M}_r(M_r, i)[j*Z:(j+1)*Z] =     M_r[h(i,j):h(i,j)+Z]
    \end{equation*}
    In words, the $j^{th}$ chunk of $i^{th}$ embedding is recovered using the chunk at the location $h(i,j)$ from $M_r$. Here, $h:\mathbf{N}^2 \rightarrow \{0,..,|M_r|\}$ is a hash function. If we set $Z=1$, then we get the mapping function for HashedNet.
\end{itemize}
We can summarize the state-of-the art embedding compression in the table \ref{tab:sota}. Our PSS theory suggests that we should be able approximate the embedding table in memory of the order of \mathcal{O(log(n)}. Thus, it is important to question if $1000\times$ compression is the best compression we can achieve on dataset like CriteoTB where we have large ($\sim$400GB sized) embedding tables. As we shall see, one of the significant roadblocks in aiming to achieve higher compression is training time. The higher the compression, the larger is the number of iterations needed to train the model to a particular quality. In the next section, we evaluate this trade-off for large DLRM model for criteo datasets. 




% It should be noted that using the sparse JLT matrices which are implemented via universal hash functions are still not very system friendly due to non-coalesced memory access patterns that are induced by sparsity. This issue was first highlighted and resolved in \cite{robez}. \cite{robez} proposed a compressed representation based on universal hashing in which chunks of embedding tables are hashed in a single array - Random Block Offset Embedding (ROBE) array. Because the basic hashed unit is a chunk, ROBE causes the memory access to be coalesced and thus making it system-friendly. \cite{robez} also proves that their way of hashing is actually theoretically better for feature hashing task. We briefly describe ROBE-Z in the PSS setup. For a complete description, we urge readers to refer to section 3 in the paper \cite{robez}. 
% \input{fig/robe_exp_figure}

% ROBE-Z divides the entire table into chunks of size Z and then hashes these chunks into a single circular array of size, say $k$. Thus in this case the memory $M_r$ is just a single array of size $k$. The mapping $\mathcal{M}$ is defined via universal hashing,
% \begin{equation*}
%     \mathcal{M}_r(M_r, i)[j*Z:(j+1)*Z] = M_r[h(i,j):h(i,j)+Z]
% \end{equation*}

% if $h(i,j) + Z$ exceeds $k$, the elements are access from the front of the circular array. Here, $h : \mathbf{N} \times \mathbf{N} \rightarrow \{0, .. k - 1\} $ is a universal hashing function with two inputs. The function can be implemented with $\mathcal{O}(1)$ memory using randomly drawn integers $A$, $B$ in the range $[1, P)$ and $C$ drawn from $[0,P)$ for large prime number $P > k$.
% \begin{equation*}
%     h(i,j) = (A*i + B*j + C) \mod P \mod k
% \end{equation*}
% The $(M_r, \mathcal{M}_r)$ describes ROBE-Z in PSS setup. The total memory of this PSS is $\mathcal{O}(|M_r|)$.  ROBE-Z style of hashing is yet another departure from the JLT-based PSS we discussed in the previous section. However, as discussed in \cite{mitzenmacher2008simple}, entropy in the data makes even simple hashing schemes work. ROBE-Z, apart from being system-friendly, has already shown the state-of-the art performance in embedding compression. Thus, we use ROBE-Z as our instance of PSS in order to evaluate the tradeoffs between system-advantage of smaller models and convergence of larger models.

==> text_nips/theory.tex <==
\label{sec:theory}
\subsection{General parameter sharing embedding table setup}
\begin{definition}[\textbf{Parameter shared setup}]
Under parameter shared setup (PSS) for embedding table of size $n \times d$, we have a set of weights $M$ and recovery function $\mathcal{M} : R^{|M|} \times \{0,..,n-1\} \rightarrow R^d$. The embedding of a token $i \in \{0,..,n-1\}$ is recovered as $\mathcal{M}(M, i)$
\end{definition}
M can be represented with any memory layout(eg. 2D/1D array). We denote the size of $M$ as $|M|$ and memory to store $\mathcal{M}$ as $|\mathcal{M}|$. Note the inherent trade-off between $|M|$ and $|\mathcal{M}|$. We can make $M$ large in order to get a very simple $\mathcal{M}$ (for example, $M{=}E$ and $\mathcal{M}(M, i){=}M[i]$) or we can keep $M$ very small at the cost of complicated $\mathcal{M}$ (for example $M$ = [0,1] and $\mathcal{M}$ combines these bits to get bit representation of $E$). An effective PSS for embedding table $E \in R^{n\times d}$ would have $(|M| + |\mathcal{M}|) \ll nd$. In context of training a PSS in an end-to-end manner, we additionally want (1) $\mathcal{M}$ is differentiable (2) $\mathcal{M}(M, i) $ computation is cheap. 

One of the key questions we want to answer that for a ground truth embedding table $E$, how small a PSS can we create? i.e. how small can $(|M| + |\mathcal{M}|)$ be. For an arbitrary $E$, it is impossible to accurately encode $E$ in sublinear memory. So, in the next section, we define a $(1 \pm \epsilon)$ PSS 
%{\color{red} For an arbitrary $E$, it is impossible to accurately encode $E$ in sublinear memory. So, in the next section, we define a $(1 \pm \epsilon)$ PSS }



%\paragraph{Notation and overloading the term ``embedding"} In literature relevant to our discussion, the term "embedding table" refers to collection of n embeddings in a tabular manner. On the ohter hand, the term "subspace embedding" \cite{woodruff} refers to a representation (a.k.a embedding) of a column space of a matrix A ( equivalently called as subspace embedding of A ). In the next section, we will talk about embedding ( like subspace embedding) for the "table". So we use the following terminology
%\begin{enumerate}
%    \item \textbf{Embedding table} to refer to collection of embeddings for $n$ points arranged in a tabular format.
%    \item \textbf{Table-space embedding} to denote embedding of the embedding table  (analogous to subspace embedding for a matrix)
%\end{enumerate}

\subsection{$(1 \pm \epsilon)$ parameter sharing setup for table $E$}
While creating an alternative representation of embedding table $E$, let us see what we would like to achieve. To start with we would like to preserve all the pairwise inner products between two embeddings of tokens from embedding table. Additionally, we also want to minimally affect the subsequent computations performed on the embeddings retrieved from the embedding table. In recommendation models, the embeddings retrieved are passed through neural network layers which will perform inner products on embeddings. With this in mind, we propose the following definition of approximate PSS for embedding table. 

\begin{definition}[$\mathbf{(1 \pm \epsilon)}$ \textbf{parameter sharing setup}]
A PSS $(M, \mathcal{M})$ is an $(1 \pm \epsilon)$ PSS for an embedding table E if the following holds, 
\begin{align*}
    & \forall x \in R^d \; \forall i \in \{ 0, .., n{-}1\} \\
    & \quad |\langle \mathcal{M}(M, i), x \rangle - \langle E[i], x \rangle | \leq \epsilon ||x||_2
\end{align*}
\end{definition}
We note that the $(1 \pm \epsilon)$ PSS for embedding table E also preserves the pairwise distances between the embeddings of different tokens as is mentioned in the following result.
\begin{theorem} \label{thm:1}
Let  $(M, \mathcal{M})$ is a $(1 \pm \epsilon)$ PSS for embedding table E, we have ,
\begin{align*}
    & \forall i, j \in \{0,...,n{-}1\}, \\
    &| \;\; || \mathcal{M}(M, i) - \mathcal{M}(M, j) ||_2 - || (E[i] - E[j]) ||_2 \; \; | \leq 2\epsilon
\end{align*}
\end{theorem}
\begin{proof}
Presented in the appendix. We first analyse the norm of recovered embedding from PSS and then extend the result to pairwise distances.
\end{proof}
Naive application of JL-Lemma will give us an existence proof of memory M of size $n\log(n)$. In the next section we show existence of M with size $dlog(n)$ which is much smaller. Also, note that the condition for $(1 \pm \epsilon)$ PSS is quite different from that of l2-subspace embedding \cite{woodruff}. As we shall see in the proof, this leads to an logarithmic dependence on n (whereas l2-subspace embeddings for $A \in R^{n \times d}$ has no dependence on n) Also, as we shall see the considerations in $(1 \pm \epsilon)$ PSS are different to those previously discussed in literature for linear algebra problems.
\subsection{$(1 \pm \epsilon)$ PSS via Johnson–Lindenstrauss Transforms}
In this section, we answer the question of how small the $|M|$ and $|\mathcal{M}|$ can be. In order to do this, we give a construction of a $(1 \pm \epsilon)$ PSS using the Johnson–Lindenstrauss Transforms(JLT) matrices. We will use the following definition of JLT matrices from \cite{woodruff}
\begin{definition}
A randomly generated matrix $S \in R^{k \times n}$ is a $JLT(\epsilon, \delta, f)$ if with probability at least $(1 - \delta)$, for any $f$-element subset $V \subset R^n$ the following holds,
\begin{equation*}
    \forall v_1, v_2 \in V \; |\langle S v_1, S v_2 \rangle  - \langle v_1, v_2 \rangle| \leq \epsilon ||v_1||_2 \, ||v_2||_2
\end{equation*}
\end{definition}
The construction of $(1 \pm \epsilon) $ PSS using JLT is presented in the following theorem,

\begin{theorem} \label{thm:2}
Let the embedding table be $E \in R^{n \times d}$. Consider a matrix $S$ which is $JLT( \epsilon / \sigma(E), \delta, 9^d + n))$ where $\sigma(E)$ denotes the maximum singular value of E. Then $M$ and $\mathcal{M}$ defined by 
\begin{align*}
    & M{=}S E \quad \mathcal{M}(M, i){=}(S e_i)^\top (M)
\end{align*}
is a $(1 \pm \epsilon) PSS$
where $e_i \in R^n$ is a one-hot encoding of integer $i$ (i.e $e_i[i] = 1$ and rest all elements of $e_i$ are 0)
\end{theorem}
\begin{proof}
The complete proof is presented in the appendix. The intuition is that we want to maintain the computations of the form $e_i^\top E x$ which can be seen as an inner product between $e_i \in R^n$ and $Ex \in R^n$. So the inner products between vectors of sets $A = \{e_0, ..., e_{n-1}\}$ and column space of $E$ need to be preserved. Once we observe this, we apply JLT to the set of n discrete points and the $1/2-net$ of column space of $E$ which contains less than $9^d$ points and get our result.
\end{proof}

Note that when using a JLT matrix S as described in theorem \ref{thm:2}, the storage cost of memory M is  $|M| = |SE| = kd$. For the mapping $\mathcal{M}$ we only need to store the matrix $S$. Thus $|\mathcal{M}| = |S|$. The cost of storing S will depend on exact choice of JLT. Since $(Se_i)$ is a $\mathcal{O}(1)$ operation as $e_i$ is a one-hot encoded vector, the cost of $\mathcal{M}(M,i)$ is just that of vector-matrix multiplication between $(Se_i)$ and $M$. Again, the exact cost depends on the choice of S. Using the random matrix formed with i.i.d normal variables, the most basic form of JLT, we can give the following bound on the memory of learnable parameters $M$

\begin{corollary}
Let E be the embedding table under consideration. Also, let $S \in R^{k \times n}$ matrix where each element of S is i.i.d $\mathcal{N}(0, \frac{1}{k})$ with k = $\Omega(\sigma^2(E) / \epsilon^2 ( log(1/\delta) + \max(d, log(n)) )$, then with a probability $(1 - \delta)$, $(M=SE, \mathcal{M}(M, i) = (Se_i)^\top (M))$ is a $(1\pm\epsilon)$ PSS for E.
\end{corollary}
Thus we obtain an upper bound on M. $|M|=\mathcal{O}(1/\epsilon^2 \max(d^2, d.log(n)) )$ when using standard normal matrix as JLT for embedding tables with bounded singular values. In this case, the mapping storage cost is $|\mathcal{M}| = kn$ as the matrix S is dense. The cost of applying $\mathcal{M}$ will be $kd$ and hence, $\mathcal{O}(1/\epsilon^2 \max(d^2, d.log(n)))$. In the next section, we will see how to reduce cost of storing $S$ in practice. This logarithmic dependence on n in the case of embedding tables with very large $n$ explains why we can achieve very high compression of 10000$\times$ for criteo-tb dataset.

\subsection{$(1 \pm\epsilon)$ PSS in practice}
\textbf{$(1 \pm \epsilon)$ PSS from a learned embedding table E}
The above discussion directly gives us an algorithm to compute a $(1 \pm \epsilon) $ of a trained embedding table $E$. We just need to compute $M=SE$ and while retrieving an embedding compute $\mathcal{M}(M,i) = (Se_i)^\top M$.
\begin{figure}
    \caption{An i
    illustration of JLT based setup of PSS, the computation involving E is performed in the sketched-space using much lesser memory of learnable parameters M. The sketching is achieved using sketching matrix S}
    \centering
    \includegraphics[scale=0.2]{fig/pss.png}
    \label{fig:pss}
    \vspace{-0.6cm}
\end{figure}


\textbf{Training end-to-end $(1 \pm \epsilon)$ PSS for embedding table E}
We can also directly train an $(1 \pm \epsilon)$ PSS in an end-to-end manner. The idea is to directly train the compressed $M$. Thus, we have a matrix of learnable weights $M \in R^{k \times d}$. Let us now look at how the forward and backward pass of embedding retrieval mapping $\mathcal{M}$ looks like
\begin{equation*}
    \mathrm{ forward(i) } = (Se_i)^\top M
\end{equation*}
The forward function takes an integer $i$ and returns a $R^{1\times d}$ array which is embedding of $i$.
\begin{equation*}
    \mathrm{ backward(i, \Delta) } =   (Se_i) \Delta
\end{equation*}
The backward pass takes in all the arguments of the forward pass along with the $\Delta \in R^{1\times d}$ which is gradients of loss with respect to output of forward pass. We can back-propagate further to $W$ using the above formulation. The result of backward pass is a $k \times d$ matrix. 

If we use a sparse $S$ such as with sparse JLT, we can achieve a sparse gradients of W. That is, only a few entries of gradient for W are non-zero. As we will see in section \ref{sec:robez_exp}, whether to propagate sparse or dense gradients is an important implementation choice. In fact, we were able to achieve better training per iteration by exploiting this choice.

\textbf{Cost considerations for PSS using JLT.} In using PSS in end-to-end training, we would be learning the memory $M$ while keeping the mapping $\mathcal{M}$ constant. Thus, unlike in sketching for linear algebra \cite{woodruff}, we care about the costs of (1) storage of learnable parameters $|M|$ (2) Cost of storing mapping $|\mathcal{M}|$, and (3) cost of computing $\mathcal{M}(M, i)$. It is clear that using standard normal JLT is not feasible due to storage of matrix S will be more expensive than storing $E$ itself! There are a lot of sparse JLT$(\epsilon, \delta, f)$ matrices S which will reduce the storage cost of $S$ \cite{achlioptas2003database,dasgupta2010sparse,kane2014sparser}.  \cite{kane2014sparser} showed that the matrix needs to have a minimum column sparsity of $\Omega(\epsilon^{-1} log( f/ \delta) log( 1/ \epsilon))$ and hence the cost of storing S while using JLT matrices is lower bounded by $\Omega(n \epsilon^{-1} log( (n + 9^d)/ \delta) log( 1/ \epsilon))$ which can still be considerably high. In the next section, we see relaxations of conditions on S for practical purposes.
